Extensive characterization of a family of efficient three-qubit gates at the coherence limit

While all quantum algorithms can be expressed in terms of single-qubit and two-qubit gates, more expressive gate sets can help reduce the algorithmic depth. This is important in the presence of gate errors, especially those due to decoherence. Using superconducting qubits, we have implemented a three-qubit gate by simultaneously applying two-qubit operations, thereby realizing a three-body interaction. This method straightforwardly extends to other quantum hardware architectures, requires only a "firmware" upgrade to implement, and is faster than its constituent two-qubit gates. The three-qubit gate represents an entire family of operations, creating flexibility in quantum-circuit compilation. We demonstrate a gate fidelity of $97.90\%$, which is near the coherence limit of our device. We then generate two classes of entangled states, the GHZ and W states, by applying the new gate only once; in comparison, decompositions into the standard gate set would have a two-qubit gate depth of two and three, respectively. Finally, we combine characterization methods and analyze the experimental and statistical errors on the fidelity of the gates and of the target states.

==> text/2theory.tex <==
\section{Theory}
\subsection{Gate Description}
There are effectively only two ways to activate any multi-qubit operation. Those being to either bring two energy levels into resonance or to supply the energy difference. Each of these operations have been shown to produce fast and high fidelity two-qubit operations. With more qubits we can induce many-body interactions by simultaneously activating couplings between shared eigenstates in the system. In our setup we activate the transitions corresponding to the individual two-qubit CZ transitions between the shared qubit, $Q_0$ and the edge qubits, $Q_1$, $Q_2$. Individually these drives would couple states $\ket{1_0 1_j}\leftrightarrow\ket{2_0 1_j}$ between qubits 0 and qubits $j=\{1,2\}$. When applied simultaneous we activate the transitions between states $\ket{110}\leftrightarrow\ket{200}\leftrightarrow\ket{101}$ where the ordering is stated in Figure 1. This creates a $\lambda$-system in the double excitation manifold. As one may notice we couple states which lie outside of the computational subspace and moreover a keen observer may note that the transitions between $\ket{210}\leftrightarrow\ket{111}\leftrightarrow\ket{201}$ are also activated at the same time and create a V-system. The timing of the interaction needs to be such that we fully remain in the computational subspace. In the double excited manifold this manifests itself as performing a full population transfer from $\ket{110}\rightarrow\ket{101}$ or in the triple excitation manifold performing a round trip from $\ket{111}$ to itself and thus acquiring a $\pi$ phase shift on the state. The net gate that performs both of these tasks is a combination of a controlled-SWAP interaction as well as a controlled-CZ interaction predicated on $Q_0$ being in its excited state. As such we denote this gate as a CCZS (Controlled CZ-SWAP). It takes the form,
\begin{equation}
    U_{CCZS}(\theta, \phi, \gamma) = \ket{0}\bra{0}_0\otimes\mathcal{I}\otimes\mathcal{I} + \ket{1}\bra{1}\otimes U_{CZS}(\theta,\phi,\gamma)
\end{equation}
with,
\begin{eqnarray}
    &&U_{CZS}(\theta, \phi, \gamma) =\\*
    && \begin{bmatrix}
                                        1 & 0 & 0 & 0 \\
                                        0 & -e^{i\gamma}\sin^2{\frac{\theta}{2}}+\cos^2{\frac{\theta}{2}} & \frac{1}{2}(1+e^{i\gamma})e^{-i\phi}\sin{\theta} & 0 \\
                                        0 & \frac{1}{2}(1+e^{i\gamma})e^{i\phi}\sin{\theta}  & -e^{i\gamma}\cos^2{\frac{\theta}{2}}+\sin^2{\frac{\theta}{2}} & 0 \\
                                        0 & 0 & 0 & -e^{-i\gamma}
                                     \end{bmatrix}\nonumber
\end{eqnarray}    
For certain parameters the unitary takes a more familiar form,
\begin{eqnarray}
    U_{CZS}(\pi/2, \phi, 0) &= \begin{bmatrix}
                                        1 & 0 & 0 & 0 \\
                                        0 & 0 & e^{-i\phi} & 0 \\
                                        0 & e^{i\phi}  & 0 & 0 \\
                                        0 & 0 & 0 & -1
                                     \end{bmatrix}
\end{eqnarray} 

Where we have a controlled SWAP-like interaction with an arbitrary phase and a CZ interaction.




==> text/5analysis.tex <==
\section{Analysis}
